Multi-Objective Optimization of Consumer Group Autoscaling in Message Broker Systems

Message brokers often mediate communication between data producers and consumers by adding variable-sized messages to ordered distributed queues. Our goal is to determine the number of consumers and consumer-partition assignments needed to ensure that the rate of data consumption keeps up with the rate of data production. We model the problem as a variable item size bin packing problem. As the rate of production varies, new consumer-partition assignments are computed, which may require rebalancing a partition from one consumer to another. While rebalancing a queue, the data being produced into the queue is not read leading to additional latency costs. As such, we focus on the multi-objective optimization cost of minimizing both the number of consumers and queue migrations. We present a variety of algorithms and compare them to established bin packing heuristics for this application. Comparing our proposed consumer group assignment strategy with Kafka's, a commonly employed strategy, our strategy presents a 90th percentile latency of 4.52s compared to Kafka's 217s with both using the same amount of consumers. Kafka's assignment strategy only improved the consumer group's performance with regards to latency with configurations that used at least 60% more resources than our approach.

==> appendices/modified_any_fit.tex <==

\section{Modified Any Fit Algorithm}


